Transcendence of the Hodge-Tate filtration

For $C$ a complete algebraically closed extension of $\mathbb{Q}_p$, we show that a one-dimensional $p$-divisible group $G/ \mathcal{O}_C$ can be defined over a complete discretely valued subfield $L \subset C$ with Hodge-Tate period ratios contained in $L$ if and only if $G$ has CM, if and only if the period ratios generate an extension of $\mathbb{Q}_p$ of degree equal to the height of the connected part of $G$. This is a $p$-adic analog of a classical transcendence result of Schneider which states that for $\tau$ in the complex upper half plane, $\tau$ and $j(\tau)$ are simultaneously algebraic over $\mathbb{Q}$ if and only if $\tau$ is contained in a quadratic extension of $\mathbb{Q}$. We also briefly discuss a conjectural generalization to shtukas with one paw.

==> macros.tex <==
%macros
\renewcommand{\AA}{\mathbb{A}}

\renewcommand\widetilde[1]{\ThisStyle{%
  \setbox0=\hbox{$\SavedStyle#1$}%
  \stackengine{-.1\LMpt}{$\SavedStyle#1$}{%
    \stretchto{\scaleto{\SavedStyle\mkern.2mu\sim}{.5467\wd0}}{.7\ht0}%
%    .2mu is the kern imbalance when clipping white space
%    .5467++++ is \ht/[kerned \wd] aspect ratio for \sim glyph
  }{O}{c}{F}{T}{S}%
}}



\newcommand{\BB}{\mathbb{B}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\TT}{\mathbb{T}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\WW}{\mathbb{W}}

\renewcommand{\det}{\mathrm{det}}
\newcommand{\lie}{\mathrm{lie}}


\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Yc}{\mathcal{Y}}

\renewcommand{\Mc}{\mathcal{M}}
\newcommand{\Vc}{\mathcal{V}}


\newcommand{\gf}{\mathfrak{g}}
\newcommand{\pf}{\mathfrak{p}}
\newcommand{\mf}{\mathfrak{m}}
\newcommand{\qf}{\mathfrak{q}}
\newcommand{\kf}{\mathfrak{k}}
\newcommand{\hf}{\mathfrak{h}}
\newcommand{\tf}{\mathfrak{t}}
\newcommand{\nf}{\mathfrak{n}}
\newcommand{\Xf}{\mathfrak{X}}

\newcommand{\tensor}{\otimes}
\newcommand{\tensorhat}{\widehat{\otimes}}

\newcommand{\cont}{\mathrm{cont}}
\newcommand{\Newt}{\mathrm{Newt}}

\newcommand{\actsonr}{\mathrel{\reflectbox{$\righttoleftarrow$}}}
\newcommand{\actsonl}{\mathrel{\reflectbox{$\lefttorightarrow$}}}

\newcommand{\isoeq}{\cong}
\newcommand{\cech}{\vee}
\newcommand{\dsum}{\oplus}

\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\Gal}{\mathrm{Gal}}
\newcommand{\sep}{\mathrm{sep}}
\newcommand{\Mod}{\mathrm{Mod}}
\newcommand{\Rep}{\mathrm{Rep}}

\newcommand{\Fil}{\mathrm{Fil}}
\newcommand{\Qlog}{\mathrm{Qlog}}
\newcommand{\Image}{\mathrm{Im}}
\newcommand{\Ker}{\mathrm{ker}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\std}{\mathrm{std}}
\newcommand{\dR}{\mathrm{dR}}
\newcommand{\Gr}{\mathrm{Gr}}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\Pic}{\mathrm{Pic}}
\newcommand{\Div}{\mathrm{Div}}
\newcommand{\Frob}{\mathrm{Frob}}
\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\Spa}{\mathrm{Spa}}
\newcommand{\Spf}{\mathrm{Spf}}
\newcommand{\Spec}{\mathrm{Spec}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\Isom}{\mathrm{Isom}}
\newcommand{\proet}{\mathrm{pro\acute{e}t}}
\newcommand{\Lie}{\mathrm{Lie}}

\newcommand{\Map}{\mathrm{Map}}
\newcommand{\Ext}{\mathrm{Ext}}

\newcommand{\GL}{\mathrm{GL}}
\newcommand{\Homc}{\mathrm{Hom}_\mathrm{cont}}


\newcommand{\height}{\mathrm{ht}}
\newcommand{\un}{\mathrm{un}}
\newcommand{\et}{\mathrm{\acute{e}t}}
\newcommand{\profet}{\mathrm{prof\acute{e}t}}
\newcommand{\an}{\mathrm{an}}
\newcommand{\cris}{\mathrm{cris}}
\newcommand{\Betti}{\mathrm{Betti}}
\newcommand{\cyc}{\mathrm{cyc}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\cl}{\mathrm{cl}}
\newcommand{\coh}{\mathrm{coh}}

\newcommand{\union}{\bigcup}

\newcommand{\rank}{\mathrm{rank}}
\newcommand{\ord}{\mathrm{ord}}
\newcommand{\Cont}{\mathrm{Cont}}
\newcommand{\Bun}{\mathrm{Bun}}
\newcommand{\piF}{\varpi_F}
\newcommand{\Irred}{\mathrm{Irred}}
\newcommand{\Sym}{\mathrm{Sym}}

\newcommand{\Ad}{\mathrm{Ad}}

\newcommand{\piE}{\varpi_E}
\newcommand{\piR}{\varpi_R}


\newcommand{\LT}{\mathrm{LT}}
\newcommand{\of}{\mathfrak{o}}
\newcommand{\Dc}{\mathcal{D}}

\newcommand{\Perf}{\mathrm{Perf}}


\newcommand{\Shperfc}{\mathrm{Sh}_{\mathrm{perf}}^*}
\newcommand{\Fl}{\mathcal{F}l}
\newcommand{\HT}{\mathrm{HT}}

\newcommand{\twistorP}{\widetilde{\PP^1_{\RR}}}

\newcommand{\Spd}{\mathrm{Spd}}

\newcommand{\End}{\mathrm{End}}
\newcommand{\Stab}{\mathrm{Stab}}
\newcommand{\GH}{\mathrm{GH}}

